Can Query Expansion Improve Generalization of Strong Cross-Encoder Rankers?

Query expansion has been widely used to improve the search results of first-stage retrievers, yet its influence on second-stage, cross-encoder rankers remains under-explored. A recent work of Weller et al. [44] shows that current expansion techniques benefit weaker models such as DPR and BM25 but harm stronger rankers such as MonoT5. In this paper, we re-examine this conclusion and raise the following question: Can query expansion improve generalization of strong cross-encoder rankers? To answer this question, we first apply popular query expansion methods to state-of-the-art cross-encoder rankers and verify the deteriorated zero-shot performance. We identify two vital steps for cross-encoders in the experiment: high-quality keyword generation and minimal-disruptive query modification. We show that it is possible to improve the generalization of a strong neural ranker, by prompt engineering and aggregating the ranking results of each expanded query via fusion. Specifically, we first call an instruction-following language model to generate keywords through a reasoning chain. Leveraging self-consistency and reciprocal rank weighting, we further combine the ranking results of each expanded query dynamically. Experiments on BEIR and TREC Deep Learning 2019/2020 show that the nDCG@10 scores of both MonoT5 and RankT5 following these steps are improved, which points out a direction for applying query expansion to strong cross-encoder rankers.

==> figures/gff.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.78\textwidth]{figures/gff_fig.pdf}
\caption{
% Our framework includes generation, filtering, and fusion to select high quality keywords for zero-shot ranking task. 
An illustration of our GFF framework. Implementation of each module (dark orange square) is introduced in Section~\ref{sec:impl}. $\alpha_i$ is the weight for combining the ranking result for each expansion in Equation~\eqref{eq:rr}.}
\label{fig:gff}
\end{figure*}

==> tables/fusion_coef.tex <==
\begin{table}[!t]
\centering
\begin{adjustbox}{max width=0.45\textwidth}
\begin{tabular}{c|ll}
\toprule
Fusion coef. &DL19 &DL20\\\midrule
0.0 &0.7514 &0.7518 \\
0.1 &\textbf{0.7528} &\textbf{0.7560}\\
0.3 &0.7514 &0.7527 \\
\qquad0.5\qquad\qquad &0.7482\qquad\qquad 
&0.7504 \\
0.7 &0.7463 &0.7433\\
0.9 &0.7453 &0.7351 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Sensitivity test of fusion coefficient on DL 19/20 based on ListwiseRankT5$_{\text{base}}$. NDCG@10 scores are reported.} 
\vspace{-3mm}
\label{tbl:fusion_coef}
\end{table}

==> tables/main_table.tex <==
\begin{table*}[!t]
\centering
% TODO: keep wiki only
% \vspace{-3mm}
% \hspace*{-1cm}
\begin{adjustbox}{max width=0.999\textwidth}
\begin{tabular}{l|ccccccccccccccccc|cc}
\toprule
\textbf{Methods}
% &DL19 
% &DL20 
& AA 
& SF 
& NQ 
& Fe 
& Qu 
& HQ 
& FQ 
& CF 
&BA 
& SD 
& T2 
&TN 
&S1 
& DB 
& NF 
&R0 
&TC 
&BEIR 
&Wiki+News\\
\midrule
ListwiseRankT5$_\text{base}$~\citep{zhuang2023rankt5}
% &0.737
% &0.736 
&0.323
&0.750
&0.565
&0.826
&0.814
&0.732
&\textbf{0.414}
&0.255
&0.541
&0.174
&0.383
&0.439
&\textbf{0.299}
&0.448
&0.375
&0.525
&\textbf{0.782}
&0.508
&0.557\\
\quad - RM3~\citep{lavrenko2001rm3}
% &0.681 
% &0.695
&\textbf{0.330}
&0.722
&0.546
&0.817
&\textbf{0.831}
&0.689
&0.377
&0.257
&0.473
&0.165
&0.360
&0.443
&0.291
&0.393
&0.358
&0.481
&0.746
&0.487
&0.539\\
\quad - query2doc~\citep{wang2023query2doc}
% &0.572 
% &0.637
&0.271
&0.671
&0.511
&0.810
&0.749
&0.640
&0.300
&0.184
&0.358
&0.140
&0.275
&0.419
&0.231
&0.367
&0.331
&0.447
&0.716
&0.437
&0.502\\
\quad - query2keyword~\citep{jagerman2023query}
% &0.690
% &0.688
&0.315
&0.739
&0.546
&0.841
&0.807
&0.725
&0.381
&0.257
&0.500
&0.168
&0.353
&\textbf{0.470}
&0.280
&0.398
&0.365
&0.496
&0.741
&0.493
&0.556\\
\quad - Ours 
% &\textbf{0.751} 
% &\textbf{0.752}
&0.324
&\textbf{0.752}
&\textbf{0.577}
&\textbf{0.846}
&0.822
&\textbf{0.744}
&0.412
&\textbf{0.261}
&\textbf{0.542}
&\textbf{0.176}
&\textbf{0.390}
&0.454
&0.292
&\textbf{0.452}
&\textbf{0.377}
&\textbf{0.541}
&0.781
&\textbf{0.514}
&\textbf{0.570}\\
\midrule
MonoRankT5$_\text{base}$~\citep{zhuang2023rankt5,nogueira2020document} 
% &0.695 
% &0.720
&0.242
&0.713
&0.553
&0.808
&0.785
&0.705
&0.364
&0.216
&0.495
&0.161
&\textbf{0.406}
&0.417
&0.286
&0.423
&0.312
&0.415
&\textbf{0.685}
&0.470
&0.519\\
\quad - RM3 
% &0.673 
% &0.693 
&\textbf{0.249}
&0.698
&0.544
&0.817
&\textbf{0.799}
&0.666
&0.354
&0.219
&0.453
&0.156
&0.390
&0.427
&\textbf{0.291}
&0.412
&\textbf{0.314}
&0.396
&0.632
&0.465
&0.511 \\
\quad - query2doc
% &0.473 
% &0.613 
&0.188
&0.640
&0.508
&0.784
&0.353
&0.594
&0.302
&0.108
&0.353
&0.127
&0.339
&0.398
&0.242
&0.368
&0.293
&0.391
&0.590
&0.392
&0.459\\
\quad - query2keyword 
% &0.672 
% &0.682 
&0.232
&0.697
&0.542
&0.828
&0.774
&0.702
&0.341
&0.215
&0.449
&0.156
&0.378
&\textbf{0.453}
&0.284
&0.397
&0.293
&0.359
&0.642
&0.455
&0.517\\
\quad - Ours 
% &\textbf{0.724} 
% &\textbf{0.730} 
&0.240
&\textbf{0.720}
&\textbf{0.569}
&\textbf{0.831}
&0.793
&\textbf{0.719}
&\textbf{0.369}
&\textbf{0.223}
&\textbf{0.499}
&\textbf{0.163}
&0.404
&0.431
&0.288
&\textbf{0.443}
&0.313
&\textbf{0.420}
&0.671
&\textbf{0.476}
&\textbf{0.532}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{NDCG@10 on BEIR.
TC=TREC-COVID, 
NF=NFCorpus, 
NQ=NaturalQuestions, 
HQ=HotpotQA, 
FQ=FiQA, 
AA=ArguAna, 
T2=Touché-2020, 
Qu=Quora, 
DB=DBPedia, 
SD=SCIDOCS, 
Fe=FEVER, 
CF=Climate-FEVER, 
SF=SciFact, 
S1=Signal-1M, 
BA=BioASQ, 
R0=Robust04, 
TN=TREC-NEWS.}
\label{tbl:main}
\vspace{-4mm}
\end{table*}
